CEBin: A Cost-Effective Framework for Large-Scale Binary Code Similarity Detection

Binary code similarity detection (BCSD) is a fundamental technique for various application. Many BCSD solutions have been proposed recently, which mostly are embedding-based, but have shown limited accuracy and efficiency especially when the volume of target binaries to search is large. To address this issue, we propose a cost-effective BCSD framework, CEBin, which fuses embedding-based and comparison-based approaches to significantly improve accuracy while minimizing overheads. Specifically, CEBin utilizes a refined embedding-based approach to extract features of target code, which efficiently narrows down the scope of candidate similar code and boosts performance. Then, it utilizes a comparison-based approach that performs a pairwise comparison on the candidates to capture more nuanced and complex relationships, which greatly improves the accuracy of similarity detection. By bridging the gap between embedding-based and comparison-based approaches, CEBin is able to provide an effective and efficient solution for detecting similar code (including vulnerable ones) in large-scale software ecosystems. Experimental results on three well-known datasets demonstrate the superiority of CEBin over existing state-of-the-art (SOTA) baselines. To further evaluate the usefulness of BCSD in real world, we construct a large-scale benchmark of vulnerability, offering the first precise evaluation scheme to assess BCSD methods for the 1-day vulnerability detection task. CEBin could identify the similar function from millions of candidate functions in just a few seconds and achieves an impressive recall rate of $85.46\%$ on this more practical but challenging task, which are several order of magnitudes faster and $4.07\times$ better than the best SOTA baseline. Our code is available at https://github.com/Hustcw/CEBin.

==> src/background.tex <==
\section{Background}

\subsection{Binary Code Similarity Detection}

Binary Code Similarity Detection (BCSD) is a technique to identify the similarities between binary code fragments, such as functions, with applications in vulnerability detection, malware classification, and code plagiarism detection. Various BCSD approaches have been investigated, including graph matching~\cite{bindiff,gao2008binhunt}, tree-based methods~\cite{pewny2014leveraging}, and feature-based techniques~\cite{farhadi2014binclone,nouh2017binsign}. Recently, deep learning techniques like Convolutional Neural Networks (CNNs)~\cite{krizhevsky2012imagenet}, Recurrent Neural Networks (RNNs)~\cite{rnn}, and Transformer-based models~\cite{devlin2018bert} have emerged as popular methods for BCSD for their accuracy and ability to learn complex features automatically.

BCSD has numerous applications, one of the most significant being software supply chain vulnerability detection. 
By identifying similarities between binary code fragments, security experts can assess if a software component is affected by known vulnerabilities, prompting necessary actions to secure the software ecosystem.

\subsection{Embedding- and Comparison-based BCSD}

In deep learning models, two primary methods can be distinguished: embedding-based and comparison-based approaches. 
Embedding-based models~\cite{feng2016scalable,xu2017neural,yu2020order,massarelli2019safe,ding2019asm2vec,jtrans,vulhawk} focus on extracting features from a function and converting them into a low-dimensional representation, or "embedding." This enables the detection of similarity based on proximity, despite differences in the original forms. One advantage of the embedding-based approach is the use of fixed representations that can be precomputed, allowing for efficient similarity detection. When calculating the similarity between a new function and existing ones, only the new function's embedding must be extracted for distance measurement. 

On the other hand, comparison-based models~\cite{li2019graph,FOSSIL,alphadiff,bindnn,shalev2018binary} involve a direct comparison between two functions. This approach typically results in higher accuracy since it accesses the raw features of each function directly. However, it requires comparing the query function to each function in the pool individually, which can be time-consuming and difficult to scale.


% In previous deep learning models, two primary methods can be distinguished: Embedding-based and Comparison-based approaches. Embedding-based models~\cite{feng2016scalable,gemini,ordermatters,massarelli2019safe,ding2019asm2vec,jtrans} extract the features of a function solely and transform each function into a low-dimensional representation, or "embedding," permitting proximity-based similarity detection despite differences in original appearances. Embedding-based approaches offer the advantage of fixed representations that can be precomputed. When calculating the similarity of a new function with existing ones, only the new function's embedding must be extracted for distance measurement, enabling efficient similarity detection. In Comparison-based models~\cite{li2019graph,FOSSIL,alphadiff,bindnn,shalev2018binary}, two functions are directly compared instead of using low-dimensional feature representations, resulting in higher accuracy as it can access the raw features of each function directly. But it requires comparing the query function with each function in the function pool one by one, yielding a poor ability to apply on a large scale.

\subsection{Pretrained Language Model}

Pre-trained language models, like Bidirectional Encoder Representations from Transformers (BERT)~\cite{devlin2018bert} and Generative Pre-trained Transformer (GPT)~\cite{radford2018improving,radford2019language,brown2020language}, have become powerful tools in natural language processing (NLP). These models employ a self-supervised training method using extensive unlabeled text data, predicting masked words and subsequent words in sentences, respectively, to achieve significant performance improvements across numerous NLP tasks. BERT and GPT excel at handling long-distance dependencies and varying output lengths, establishing themselves as state-of-the-art in many applications.

In tasks such as binary code semantic similarity detection (BCSD), researchers~\cite{vulhawk,yu2020order,jtrans} have widely adopted BERT for its robust feature extraction capabilities. As a result, Transformer-based models have become the de facto SOTA for these tasks. Further performance improvements can be achieved by integrating Transformer-based models with Graph Neural Networks (GNNs) to leverage structural information present in the data. Empirical studies suggest that these hybrid models surpass traditional deep learning techniques, including Convolutional Neural Networks (CNNs) and Recurrent Neural Networks (RNNs), in terms of overall performance.

% \subsection{Binary Code Similarity Detection} 
% Binary Code Similarity Detection (BCSD) is a technique to determine whether two binary code fragments, such as functions, are similar or homologous. The goal is to identify similarities between binary codes for various applications, like vulnerability detection, malware classification, and code plagiarism detection. \qiuhan{applications or tasks?}
% Several approaches for BCSD have been investigated, including non-deep learning methods such as graph matching~\cite{bindiff,gao2008binhunt}, tree-based approaches~\cite{pewny2014leveraging}, and feature-based techniques~\wh{to cite}. In recent years, deep learning techniques like Convolutional Neural Networks (CNNs)~\cite{krizhevsky2012imagenet}, Recurrent Neural Networks (RNNs)~\cite{massarelli2019safe}, and Transformer-based models~\cite{devlin2018bert} have emerged as popular methods for BCSD due to their ability to automatically learn complex features and deliver high accuracy. 
% Recently, Transformer-based models have become a de facto state-of-the-art approach for BCSD. 
% These models offer several advantages, including a strong capacity for capturing long-range dependencies and dealing with variable-length input sequences. 
% Transformer-based methods can also be combined with Graph Neural Networks (GNNs)~\cite{yu2020order} to exploit structural information, further enhancing their performance. 
% Several studies have demonstrated the superior performance of these models compared to traditional deep learning techniques like CNNs and RNNs~\wh{to cite}.

% The methods utilizing deep learning networks contain two main approaches

% \subsubsection{Embedding-based}

% \subsubsection{Comparison-based}

% \subsection{Challenges in Existing BCSD Solutions} 
% Existing BCSD solutions face several challenges, including:

% \begin{packeditemize} 

% \item \textbf{Migrating to new scenarios:} Many BCSD techniques struggle to generalize across new scenarios due to the significant variations in semantically identical or similar binary code. These variations can arise from differences in compiler optimizations or Instruction Set Architectures (ISAs). As a result, it is often necessary to retrain models with new data when faced with an unfamiliar environment or a change in ISA.

% \item \textbf{Large function pool size:} BCSD models typically perform well with small function repositories, but their performance declines as the pool size increases. Current BCSD solutions face scalability issues, as they require significant computation resources to search for potential vulnerabilities in large-scale function pools~\cite{jtrans}. To improve recall and precision when dealing with a large pool size, one must balance the trade-off between computation cost and search performance.

% \end{packeditemize}

% \subsection{Pre-trained Language Model}


% \subsection{BCSD for Vulnerability Detection Task} 
% BCSD has numerous applications, one of the most significant being software supply chain vulnerability detection. 
% By identifying similarities between binary code fragments, security experts can assess if a software component is affected by known vulnerabilities, prompting necessary actions to secure the software ecosystem.

% However, there is a lack of a widely recognized benchmark to evaluate the performance of vulnerability search techniques using various BCSD approaches. 
% The limited number of vulnerabilities in existing benchmarks and the variable vulnerabilities and software considered in each study make it difficult to conduct a fair comparison and accurately evaluate different solutions. 
% Furthermore, these methods typically measure only accuracy, neglecting recall, which is equally important in software supply chain vulnerability detection.

% To address these issues, it is imperative to develop a more comprehensive and standardized benchmark for assessing the effectiveness of BCSD methods in the context of software supply chain vulnerability search.
